Multi-view Self-supervised Disentanglement for General Image Denoising

With its significant performance improvements, the deep learning paradigm has become a standard tool for modern image denoisers. While promising performance has been shown on seen noise distributions, existing approaches often suffer from generalisation to unseen noise types or general and real noise. It is understandable as the model is designed to learn paired mapping (e.g. from a noisy image to its clean version). In this paper, we instead propose to learn to disentangle the noisy image, under the intuitive assumption that different corrupted versions of the same clean image share a common latent space. A self-supervised learning framework is proposed to achieve the goal, without looking at the latent clean image. By taking two different corrupted versions of the same image as input, the proposed Multi-view Self-supervised Disentanglement (MeD) approach learns to disentangle the latent clean features from the corruptions and recover the clean image consequently. Extensive experimental analysis on both synthetic and real noise shows the superiority of the proposed method over prior self-supervised approaches, especially on unseen novel noise types. On real noise, the proposed method even outperforms its supervised counterparts by over 3 dB.

==> functions/figures.tex <==

\newcommand{\plotfigure}[3]{       
\includegraphics[width=0.3\textwidth]{#1}
% \caption*{#2(#3)}
}



==> sections/blocks/table_metrics.tex <==



\begin{table}[h]
	\caption{{Feature Consistency Metric
(FCM)  Measurement}}
\vspace{0.2cm}
	\small
	\centering
	% \resizebox{\linewidth}{!}{
	\setlength{\tabcolsep}{4pt}
	%\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{c|cccccc}
     \toprule
     
     % First Line  \multirow{}{}   \makecell[c]{ 
     Method  & DnCNN 
      & N2N  & R2R & LIR & OurB & Our \\
     \midrule
     FCM & 0.87 & 0.81 & 0.79 & & & 0.76
      \\  
     \bottomrule
    \end{tabular}%
	% }
	\label{tab:fcm}
\end{table}



==> sections/blocks/table_models.tex <==
\begin{table}[h]
	\caption{{Quantitative comparison of different methods on BSD68 test set (Will be update at Nov 9.).}}
 \vspace{0.2cm}
	\small
	\centering
	% \resizebox{\linewidth}{!}{
	\setlength{\tabcolsep}{4pt}
	%\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{cccc}
     \toprule
     
     % First Line  \multirow{}{}   \makecell[c]{ 
     \multirow{2}{*}{Method} & \multirow{2}{*}{Network} & Benchmark & Benchmark \\
     & & PolyU \cite{xu2018real} & CC \cite{nam2016holistic}
      \\
      \midrule
      Baseline, N2C & DnCNN  & 35.60/0.964 & 33.47/0.932  \\
      Baseline, N2N & DnCNN \\
     \midrule
     CBM3D & -    & 37.01/0.944 & 35.19/0.858\\
     S2S & DnCNN & 37.48 /0.950 &   37.56/0.947 \\
     DIP & U-Net & 36.95/0.940 & 37.12/0.932\\
     N2V & DnCNN & 33.83/0.873 & 32.20/0.854\\
     N2S & DnCNN & 35.04/0.902  & 33.41/0.850 \\
     R2R & DnCNN & 38.47/0.965 &  37.78/0.951 \\
     LIR & AE   \\
     LIR & DnCNN  \\
     Ours & AE   \\
     Ours & DnCNN  \\
     Ours & Swin-T  \\
     \midrule
    %   & 15  & 31.04 
     \\ \bottomrule
    \end{tabular}%
	% }
	\label{tab:DPD_Noisier}
\end{table}

==> sections/blocks/table_result.tex <==
% \jb{

\begin{table*}[!t]
\label{tab:qutitative}
	\caption{Quantitative comparison of different methods on BSD68 test set.please highlight the best performed results. also include the SSIM. The best PSNR(dB)/SSIM results among denoising methods without the need for clean images are marked in \textbf{bold}. \ch{This table shows PSNR/SSIM of methods trained on fixed Sigma/ Variational Sigma and test on BSD68 dataset}}
 % ∗ denotes that results are obtained from the website
% of SIDD Benchmark}
        \vspace{0.2cm}
	\small
	\centering
	% \resizebox{\linewidth}{!}{
	\setlength{\tabcolsep}{4pt}
 
	%\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{c|c|cc|ccc|ccc|ccc}
     \toprule
     
     % First Line  \multirow{}{}   \makecell[c]{ 
     \multirow{2}{*}{Training} & \multirow{2}{*}{Test $\hat \sigma$} & \multicolumn{2}{c|}{Single-image-based} & \multicolumn{3}{c|}{Noisy/ Clean} &
     \multicolumn{3}{c|}{Noisy/ Noisy}  &\multicolumn{3}{c}{Invariant Feature} 
      \\
    %  \midrule
      & & BM3D  & DIP &  AE & DnCNN & DBD 
      & N2N & N2S &  R2R & LIR & Our(AE) & Our(Swin) \\
    
     \midrule
      \multirow{3}{*}{BSD68 }     
      & 15  & 31.04  & 30.23 & 31.03 & 31.73 & 31.43 & 30.12  & 29.99  &30.73  & 29.84 & 32.02 & 32.67  \\  
      & 25  & 28.56  & 27.96  & 28.71 & 29.23 & 29.02  & 28.33 & 28.12 &  29.01  & 27.90 & 29.34 & 29.88
      
      \\
     & 50   & 25.60 &25.04  & 26.01 &  26.42 & 26.10  & 25.42 & 25.62 &  %  R2R & LIR & OurB & Our 
     25.66 &  24.78 & 26.40 & 26.61
     \\ 
     & 75   & 24.21 & 23.78 & 24.32 & 24.67 &  24.45  & 24.50 & 24.21  & 24.49
    %  LIR & OurB & Our 
    &  24.07  &      24.56    & 24.78 
     
     \\
    %  \midrule
    %  \midrule
    % ---------------------- Color
     % First Line  \multirow{}{}   \makecell[c]{ 
     \midrule
      \multirow{4}{*}{Color BSD68 }     
      %      BM3D   & S2S & DIP & DnCNN & MWCNN 
      & 15  & 33.48 & 30.82 &  33.13 & 33.48 & 33.59
      %  N2N & N2V & N2S & R2R & LIR & OurB & Our 
           &  32.54  &  32.23  &  32.95  &  30.96  &  32.66  & 33.53
      \\  
      & 25  & 30.71 &  28.53    & 30.42
      %  N2N & N2V  & R2R & LIR & OurB & Our 
      &   31.10 & 30.78 & 30.20   &  29.78 & 30.23 &  28.76  & 30.33 & 30.91
      \\
      & 50  & 27.36     &  26.67   &   27.52
      %  N2N & N2V & N2S & R2R & LIR & OurB & Our 
      & 27.88 & 27.43 & 27.47  & 27.32  & 27.15 &  25.37   &   27.47   & 28.05
          \\
    % & & BM3D & S2S & DIP &  CNN & DnCNN
      & 75  & 25.34   &  22.53   & 25.22  &   25.91 & 25.52
      %  N2N & N2V & N2S & R2R & LIR & OurB & Our 
      &   25.63   &  25.03  &  25.39  &  24.48  &  25.70  & 26.32
          \\
     
     \bottomrule
    \end{tabular}
	
	
\end{table*}

==> sections/images/mbm.tex <==
%---------------------------------
\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{img/bfm.jpg} 
   \caption{Here is an explanation of Bernoulli Feature Mixture}
   \label{fig:bfm}
\end{figure}
%---------------------------------




==> sections/tables/unseen.tex <==
\begin{table}[h]
	\caption{AVG Test results of Model Trained on Gaussian @ [5,50] on Unseen Noise}
 \vspace{0.2cm}
	\small
	\centering
	% \resizebox{\linewidth}{!}{
	\setlength{\tabcolsep}{4pt}
	%\renewcommand{\arraystretch}{0.98}
    \begin{tabular}{cccc}
     \toprule
     
     % First Line     \makecell[c]{ 
     \multirow{2}{*}{Method} & Poisson & Speckle & Salt-and-Pepper \\
      & $\lambda \in [5, 50]$ & $ v \in [25, 50]$ & $r \in [0.3, 0.5]$\\
      \midrule
      Baseline, N2C &  40.49/0.97 & 33.32/0.89 & 28.85/0.82  \\
      
     \midrule
     N2N  & 41.35/0.97 & 00.00/0.00 & 28.59/0.8  \\
     N2N (MeDia)  & 41.35/0.97 & 00.00/0.00 & 28.59/0.8  \\
     N2S  & 00.00/0.00 & 00.00/0.00 & 00.00/0.00 \\
     R2R  & 00.00/0.00 & 00.00/0.00 & 00.00/0.00   \\
     LIR & 00.00/0.00 & 00.00/0.00 & 00.00/0.00   \\
     MeDia & 00.00/0.00 & 00.00/0.00 & 00.00/0.00 
     \midrule
    %   & 15  & 31.04 
     \\ \bottomrule
    \end{tabular}%
	% }
	\label{tab:DPD_Noisier}
\end{table}

==> tables/im.tex <==
\begin{table}[h]
	\caption{ Average PSNR(dB)/SSIM of inpainting results on Set11. The best PSNR is in \textbf{bold}. S2S and DIP are trained and tested on the same single image. While MeD  is trained with \textit{Corruption Pool} contains noises, down-scalings and inpainting mask. }
	\label{tab:im}
 \vspace{0.2cm}
	\small
	\centering
	% \resizebox{\linewidth}{!}{
	\setlength{\tabcolsep}{4pt}
	%\renewcommand{\arraystretch}{0.98}
 \resizebox{0.49\textwidth}{!}{
    \begin{tabular}{c|ccc}
     \toprule
   Dropping Ratio & DIP \cite{ulyanov2018deep} &  S2S \cite{quan2020self2self} &  MeD (Ours)\\
    \midrule
50\% & 33.45/ 0.9217 & {34.91/ 0.9479} & \textbf{36.24/ 0.9617} \\
70\% & 28.53/ 0.8501 & {30.94/ 0.8845} & \textbf{31.05/ 0.9161} \\
90\% & 24.39/ 0.7360 & {25.97/ 0.7933} & \textbf{26.01/ 0.8052} \\

 \bottomrule
    \end{tabular}%
    }
	% }
\end{table}
% \vspace{-0.5}
